Text-driven Adaptation of Foundation Models for Few-shot Surgical Workflow Analysis

Purpose: Surgical workflow analysis is crucial for improving surgical efficiency and safety. However, previous studies rely heavily on large-scale annotated datasets, posing challenges in cost, scalability, and reliance on expert annotations. To address this, we propose Surg-FTDA (Few-shot Text-driven Adaptation), designed to handle various surgical workflow analysis tasks with minimal paired image-label data. Methods: Our approach has two key components. First, Few-shot selection-based modality alignment selects a small subset of images and aligns their embeddings with text embeddings from the downstream task, bridging the modality gap. Second, Text-driven adaptation leverages only text data to train a decoder, eliminating the need for paired image-text data. This decoder is then applied to aligned image embeddings, enabling image-related tasks without explicit image-text pairs. Results: We evaluate our approach to generative tasks (image captioning) and discriminative tasks (triplet recognition and phase recognition). Results show that Surg-FTDA outperforms baselines and generalizes well across downstream tasks. Conclusion: We propose a text-driven adaptation approach that mitigates the modality gap and handles multiple downstream tasks in surgical workflow analysis, with minimal reliance on large annotated datasets. The code and dataset will be released in https://github.com/CAMMA-public/Surg-FTDA

==> intro_bkp.tex <==
Surgical workflow analysis is a critical task to enable intelligent computer-assisted intervention systems \citep{maier2022surgical, padoy2019machine}, and it has been an active area of research in recent years. It requires precise surgical scene understanding and human intent anticipation to provide peripheral assistance feedback to surgeons. Early approaches, due to the lack of sufficient data, rely heavily on feature engineering, incorporating semantic features~\citep{twinanda2016endonet}, surgical scene interaction information~\citep{yuan2022anticipation,murali2023latent}, and other domain-specific knowledge to improve scene understanding. With the rise of deep neural networks and the availability of annotated datasets, recent methods have shifted toward designing architectures that better capture temporal dependencies \citep{czempiel2020tecno,gao2021trans} and other complex features. While these architectures have led to notable improvements, they often exhibit limited generalizability and require large amounts of paired image-label data for training, limiting their scalability. We address these challenges by leveraging emerging surgical foundation models for surgical workflow analysis, framing both discriminative and generative tasks as a text generation problem. Specifically, we perform few-shot data selection to obtain minimal supervision from the unlabeled downstream dataset and then train a text decoder using a text-driven adaptation strategy. This approach significantly reduces the reliance on large paired image-label datasets while ensuring robust performance and providing a scalable, data-efficient solution.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{model_archiv3.drawio.pdf} 
    \caption{(a) Conventional adaptation of multi-modal foundation model requires paired image-label data for training; (b) Our text-driven adaptation of the foundation model does not require a large number of image-label pairs to achieve the surgical workflow analysis.}
    \label{fig:fig1}
\end{figure}

Surgical multi-modal foundation models \citep{yuan2023learning, yuan2024hecvl} are pre-trained on a large corpus of vision-language entities, aligning semantically similar images, videos, and text. These models demonstrate good generalizability, enabling adaptation to various surgical procedures and tasks, such as triplet recognition \citep{nwoye2021rendezvous}, and visual question answering \citep{seenivasan2022surgical,yuan2024advancing}. Conventionally, as shown in Fig.~\ref{fig:fig1} (a), pre-trained visual and textual encoders are adapted to downstream class labels through prompt tuning \citep{zhou2022conditional,yao2023visual} or fine-tuning \citep{wang2021actionclip}. However, this approach relies heavily on annotated image-label data, which is expensive and limited to specific vocabulary, preventing open-vocabulary generative tasks like image captioning~\citep{russakovsky2015imagenet}.

To overcome these limitations, we propose Surg-FTDA, a few-shot text-driven adaptation approach that transfers the pre-trained surgical multi-modal foundation model to various surgical workflow analysis tasks using minimal paired image-label data, as shown in Fig.~\ref{fig:fig1} (b). We perform the adaptation in two stages. In the first stage, we select a few data anchors (images from the downstream dataset) based on the distribution in the visual embedding space using methods such as KMeans clustering, ensuring coverage of key visual features. Along with the anchors' paired labels, we perform text-driven training while reducing the modality gap inherent in the pretraining process of surgical foundation models. This gap arises when vision and text embeddings are clustered separately, leading to situations where semantically dissimilar images are closer to each other than their corresponding texts \citep{liang2022mindgapunderstandingmodality}. While recent approaches, such as CapDec \citep{nukrai2022text} and CLOSE\citep{gu2023can}, introduced Gaussian-based noise injection to reduce the modality gap for text-driven training, they often compromise cross-modal correspondence information and neglect the geometric structure of the embedding space. Our approach addresses these issues by leveraging the selected few-shot data anchors to learn a transformation between visual and textual modalities. This process ensures proper alignment between the modalities while maintaining the semantic and geometric structure of the embedding space. 

Unlike conventional adaptation strategies, our text-driven training approach does not require paired image-label data for the target tasks, making the process more efficient and scalable. Moreover, we construct a single text decoder for multiple workflow analysis tasks, demonstrating the foundation model's versatility in downstream tasks. We summarize our main contributions as follows:
\begin{itemize} 
    \item We propose a few-shot text-driven adaptation approach to transfer surgical multi-modal foundation models to various surgical workflow analysis tasks with minimal paired image-label data. 
    \item We address the modality gap by performing few-shot data selection and modality alignment, which selects a small number of data anchors to learn a transformation matrix between visual and textual modalities, preserving cross-modal correspondence. 
    \item We show that our method generalizes well across both discriminative and generative tasks in surgical workflow analysis, reducing the reliance on large-scale annotated datasets. 
\end{itemize}

